Bridge Simulation and Metric Estimation on Lie Groups and Homogeneous Spaces

We present schemes for simulating Brownian bridges on complete and connected Lie groups and homogeneous spaces. We use this to construct an estimation scheme for recovering an unknown left- or right-invariant Riemannian metric on the Lie group from samples. We subsequently show how pushing forward the distributions generated by Brownian motions on the group results in distributions on homogeneous spaces that exhibit non-trivial covariance structure. The pushforward measure gives rise to new parametric families of distributions on commonly occurring spaces such as spheres and symmetric positive tensors. We extend the estimation scheme to fit these distributions to homogeneous space-valued data. We demonstrate both the simulation schemes and estimation procedures on Lie groups and homogenous spaces, including $\SPD(3) = \GL_+(3)/\SO(3)$ and $\mathbb S^2 = \SO(3)/\SO(2)$.

==> Content/Abstract.tex <==
\begin{abstract}
Computing sample means on Riemannian manifolds is typically computationally costly as exemplified by computation of the Fréchet mean which often requires finding minimizing geodesics to each data point for each step of an iterative optimization scheme. When closed-form expressions for geodesic are not available, this leads to a nested optimization problem which is costly to solve. The impact is particularly emphasized in geometric deep-learning, particularly Riemannian convolutional neural networks, where a weighted Fréchet mean enters each layer of the network, potentially requiring an optimization in each layer. The weighted diffusion mean offers an alternative to the weighted Fr\'echet mean. We show how the diffusion mean and weighted diffusion mean can be estimated with a simulation scheme that does not require nested optimization. We achieve this by conditioning a Brownian motion in a product manifold to hit the diagonal at a predetermined time. We develop the theoretical foundation for the sampling based mean estimation, we implemente a numerical simulation scheme, and we demonstrate the applicability of the method with examples of sampled means on several manifolds. 

\keywords{Fréchet Mean, Diffusion Mean, Bridge Simulation, Geometric Statistics}
\end{abstract}

==> Content/Background.tex <==
\section{Background}
We here survey the necessary concepts from Riemannian geometry, geometric statistics and stochastic analysis necessary for the remainder of the paper.


\input{Content/Sub-content/riemannian_geometry}

\input{Content/Sub-content/wFM}

\input{Content/Sub-content/wDM}

\input{Content/Sub-content/bridges}

\input{Content/Sub-content/manifold_diffusions}

\input{Content/Sub-content/riemannian_bridges}

==> Content/Bridge_for_mean_approximation.tex <==
\section{Diffusion Mean Estimation}
We now use the bridge sampling techniques described above to estimate the diffusion mean \eqref{eq:wdiffusionmean} by sampling.
%Convolutional networks for manifold valued data is a subbranch of geometric deep learning pioneered by Bronstein et al. \cite{bronstein2017geometric}. Within each layer of the convolutional network the weighted Fréchet mean is evaluated \cite{chakraborty2018manifoldnet, chakraborty2020manifoldnet}. Such a task computationally heavy as the Fréchet mean requires calculation of geodesics. Sommer and Bronstein \cite{sommer2020horizontal} proposed an alternative to the (weighted) Fréchet mean estimator, namely the weighed diffusion-mean. Approximations of the diffusion-mean can be done via bridge sampling as was done by the authors \cite{jensen2021simulation}. 
The setup for diffusion mean estimation described in the literature (e.g. \cite{sommer_brownian_2017}) is as follows: Given a set of observations $x_1,\dots,x_n \in M$, we can for each observation sample a guided bridge process $X_{t,i}|(X_{0,i} = X_0^i, X_{T,i} = x_i)$ conditioned on $x_i$ with random initial points $X^i_0$. By means of Monte Carlo sampling, the expectation over the correction factors can be computed and hence the transition density can be evaluated using \eqref{eq: transition density estimate}. An iterative maximum likelihood approach using gradient descent in turn yields an approximation of the diffusion-mean. In each iteration, the starting point of each guided bridge process becomes the maximum likelihood estimate of the previous iteration. The computation of the diffusion-mean, in the sense just described, is, similarly to the Fréchet mean, computationally expensive. 

We here explore the idea put forth in \cite{sommer2020horizontal}: We turn the situation around to simulate $n$ independent Brownian motions starting at each of $x_1,\ldots,x_n$. We now condition the $n$ processes to coincide at time $T$. We will show that the value $x_{1,T}=\cdots=x_{n,T}$ is an estimator of the diffusion mean. By introducing weights in the conditioning, we can similarly estimate the weighted diffusion mean. The construction can concisely be described as a single Brownian motion on the $n$-times product manifold $M^n$ conditioned to hit the diagonal $\{(x,\ldots,x)|x\in M\}\subset M^n$. We start with an example to motivate the construction.

\begin{example}
    Recall the following basic fact from Euclidean space.
    Consider the two-dimensional multivariate normal distribution 
    \begin{equation*}
    \begin{pmatrix}
        X\\Y
        \end{pmatrix}
        \sim
        N\left(
        \begin{pmatrix}
        \mu_1\\ \mu_2
        \end{pmatrix}
        ,
        \begin{pmatrix}
        \sigma_{11} \quad \sigma_{12}\\\sigma_{21} \quad \sigma_{22}
        \end{pmatrix}
        \right).
    \end{equation*}
The conditional distribution of $X$ given $Y=y$ follows a univariate normal distribution
    \begin{equation*}
        X|Y=y \sim N\left(\mu_1 + \sigma_{12}\sigma_{22}^{-1}(y-\mu_2), \sigma_{11}-\sigma_{12}\sigma_{22}^{-1}\sigma_{21}\right).
    \end{equation*}
The proof of the above statement relies on the fact that if $X \sim N\left(\mu, \Sigma\right)$, then for any linear transformation $AX + b \sim N\left(b + A\mu, A \Sigma A^T\right)$. Defining the random variable $Z= X-\sigma_{12}\sigma_{22}^{-1}Y$, the result above applied to $(Z,X)$ will show that $Z \sim N\left(\mu_1 - \sigma_{12}\sigma_{22}^{-1}\mu_2, \sigma_{11}-\sigma_{12}\sigma_{22}^{-1}\sigma_{21}\right)$. The conclusion then follows from $X= Z +\sigma_{12}\sigma_{22}^{-1}Y$. Note that $X$ and $Y$ are independent if and only if $\sigma_{12}=\sigma_{21}=0$ and the conditioned random variable is identical in law to $X$.
\end{example}

Let now $x_1, \dots, x_n \in M$ be observations and let $x = (x_1, \dots, x_n) \in M^n$ be an element of the $n$-product manifold $M \times \dots \times M$ with the product Riemannian metric. We again first consider the case $M=\mathbb R^d$:

\begin{example}
    Let $Y_i \sim N\left(x_i, Tw^{-1}_i I\right)$ be independent random variables. The conditional distribution $Y_1|Y_1= \dots =Y_n$ follows a normal distribution given by $N\left( \frac{\sum_i w_i x_i}{\sum_i w_i},\frac{T}{\sum_i w_i}\right)$. This can be seen inductively:   
    The conditioned random variable $Y_1 | Y_1 = Y_2$ is identical to $Y_1 | Y_1-Y_2 = 0$. Now let $X = Y_1$ and $Y = Y_1-Y_2$ and refer to Example 1.
    In order to conclude, assume $Z_n := Y_1|Y_1 = \cdots, = Y_{n-1}$ follow the desired normal distribution. Then $Z_n|Z_n = Y_n$ is normally distributed with the desired parameters and $Z_n|Z_n = Y_n$ is identical to $Y_1|Y_1=\cdots = Y_n$.
\end{example}

The following example establishes the weighted average as a projection onto the diagonal.

\begin{example}
    Let $x$ be a point in $\R^{nd}$ and let $u \in \R^{nd}$ be the vector spanning the diagonal, i.e., $u$ is the vector of ones. Let $e = u/\lVert u \rVert$, then the orthogonal projection of $x$ onto the diagonal is the vector $\langle x, e\rangle e = \left(\frac{1}{nd} \sum_{i=1}^{nd} x_i \dots \frac{1}{nd} \sum_{i=1}^{nd} x_i\right)^T$. From this, we see that the orthogonal projection onto the diagonal yields the arithmetic mean of the coordinates. This is illustrated in Fig. \ref{fig: projection onto diagonal}.
\end{example}

\begin{figure}
\centering
\def\svgwidth{0.3\textwidth}
\input{mean_on_diagonal_densities.eps_tex}
\caption{The mean estimator viewed as a projection onto the diagonal of a product manifold. Conditioning on the closest point in the diagonal yields a density on the diagonal depending on the time to arrival $T>0$. As $T$ tends to zero the density convergence to the Dirac-delta distribution (grey), whereas as $T$ increases the variance of the distribution increases (rouge).}\label{fig: projection on diagonal with density}
\end{figure}

%\subsection{Guided Bridges to Submanifolds}

%In the remainder of the paper, we focus on the idea developed in \cite{sommer2020horizontal} 
%by reversing the conditioning, i.e., by sampling the conditioned process $X_t|(X_0^i = x_i, X_{T,1}=\cdots = X_{T,n})$ on the product manifold $M^n := M \times \cdots \times M$, where each coordinate process is initiated from the observed data points. 

%We now use these examples but on manifolds: We sample the mean by sampling from the conditional distribution $Y_1|Y_1=\dots=Y_n$ from example 2 using a guided proposal scheme on the product manifolds $M^n$ and on each step of the sampling projecting to the diagonal as in examples 3. To make this precise, we first show the relation between the Fermi bridges \cite{thompson2015submanifold, thompson2018brownian} and the guided bridges conditioned on the diagonal of a product manifold. Let $M^n$ be the product manifold endowed with the product connection $\nabla^{M^n} = \nabla^M \times \cdots \times \nabla^M$. The following result establishes the diagonal of $M^n$ with the product connection as a totally geodesic submanifold of $M^n$.

%\begin{proposition}\label{result: totally geodesic}
%    Let $M^n$ be endowed with the connection $\nabla^{M^n}$, then the diagonal map $x \mapsto (x,\dots,x)$ embeds $M$ as a totally geodesic submanifold of $M^n$.
%\end{proposition}
%
%\begin{proof}
%    This follows by a similar reasoning as the proof of \cite[Proposition 2.6.10]{hsu2002stochastic}.
%\end{proof}
%
%As an immediate consequence of the above proposition, the diagonal $\diag(M^n)$ is a totally geodesic submanifold of $M^n$.
%
%\begin{corollary}\label{result: totally geodesic corollary}
%    The diagonal $\diag(M^n)$ is a totally geodesic submanifold of $M^n$.
%\end{corollary}




    
    
    
\subsection{Bridges to Diagonal}

The idea of conditioning diffusion bridge processes on the diagonal of a product manifold originates from the facts established in example 2 and example 3. 
We sample the mean by sampling from the conditional distribution $Y_1|Y_1=\dots=Y_n$ from example 2 using a guided proposal scheme on the product manifolds $M^n$ and on each step of the sampling projecting to the diagonal as in examples 3. 
The simulation scheme of these bridge processes yields method to sample from a distribution of the diffusion mean on the diagonal as shown in Fig. \ref{fig: projection on diagonal with density}.



%Let $dU_t =  H_i(U_t) \circ dW^i_t$ be a Brownian motion on $FM^n$ and let $X_t=\pi(U_t)$ be the corresponding Brownian motion on the product manifold $M^n$. 
%The stochastic differential equation for a diffusion bridge $X_t$ on $M$ conditioned at $X_T = v$, for some $v \in M$, is a solution to 
%    \begin{equation}
%    \begin{split}
%        dU_t = & H_i(U_t) \circ \left(dB^i_t + H_i \log \tilde p_{T-t}(U_t, v) dt\right), \\
%        dX_t = &d\pi(U_t)
%    \end{split}
%    \end{equation}
%where $\tilde p_t(u,v) = p_t(\pi(u),v)$ is the lift of the transition density of the Brownian motion on $M$. With $\Pb$ denoting the measure of a Brownian motion, by Girsanov's theorem (see \cite[Chapter 4, Proposition 1B]{elworthy1988geometric}), the Radon-Nikodym derivative $d\Pb_{x,v}/d\Pb$ is given by 
%    \begin{equation}
%        \frac{d\Pb_{x,v}}{d\Pb}|_{\cF_t}
%        =
%        e^{\int_0^t \left\langle \nabla \log p_{T-s}(X_s,v), U(e_i) \right\rangle dW^i_t - \frac{1}{2} \int_0^t \lVert \nabla \log  p_{T-s}(X_s,v) \rVert^2 ds},
%    \end{equation}
%where $\langle \nabla f, u(e_i)\rangle dw^i := \langle \nabla f, u\circ dw\rangle$ (see also Hsu \cite{hsu2002stochastic} for a detailed derivation). The relation with equation \eqref{eq: doob's transform} is evident. 
%

\iffalse
As is often the case, in Euclidean spaces and on manifolds, the transition densities are intractable. We state a version of the Girsanov-Cameron-Martin formula:
\begin{theorem}\label{thm: general girsanov}
Let $X$ be a diffusion process on $M$ started at $x \in M$ with elliptic generator $\mathcal A$. Assume that $X$ is non-explosive. For any measurable vector field $c_t$ on $M$ satisfying, for $T > 0$,  $\int_0^T \lVert c(s,X_s)\rVert^2 ds < \infty $, $\Pb$-a.s.., we can define a measure $\Pb^c_t$ on $\cF_t$, for $t\in[0,T]$, by (NEEDS TO BE A MARTINGALE)
    \begin{equation}
        \frac{d\Pb^{c}}{d\Pb}\bigg|_{\cF_t}(X) = \exp\left\{\int_0^t \left\langle c(s,X_s), U_s(e_i) \right\rangle dZ^i_s - \frac{1}{2} \int_0^t \lVert c(s,X_s) \rVert^2 ds\right\}.
    \end{equation}
If $\frac{d\Pb^{h}}{d\Pb}|_{\cF_t}(X)$ is martingale with initial value of one, the measure $\Pb^h$ is a probability measure. Under the new measure $\Pb^h$, $X$ is a diffusion process with generator $\mathcal A  + h_t$.
\end{theorem}    

\begin{corollary}
Let $X$ be a Brownian motion with drift started at $x \in M$, i.e., $\mathcal A = \frac{1}{2}\Delta + V$. Assume that $X$ is non-explosive and that $V$ is a locally bounded and measurable vector field on $M$. With the same assumptions on $h_t$ as in \refthm{thm: general girsanov}, we get that under $\Pb^h$, $X$ is a Brownian motion with drift $V+h_t$.
\end{corollary}

From the Girsanov-Cameron-Martin formula above it is clear that any

\fi



\iffalse
\subsubsection{Girsanov's Transform on Product Manifold}


Let $Y$ be a process on the product manifold $M^n = M_1 \times \dots \times M_n$. Let $\pi_j \colon M^n \rightarrow M_j$ be the canonical projections, for each $j$. We can introduce a Riemannian metric on $M^n$ as follows
    \begin{equation*}
        \left\langle u,v \right\rangle_p = \left\langle d\pi_1(u), d\pi_1(v) \right\rangle_{p_1} + \dots +  \left\langle d\pi_n(u), d\pi_n(v) \right\rangle_{p_n},
    \end{equation*}
for all $p = (p_1,\dots,p_n) \in M^n$ and $u,v \in T_p M^n$.
    \begin{lemma}\label{lemma: Laplace-beltrami on product}
        With the above Riemannian metric structure, the Laplace-Beltrami operator on $M^n$ satisfy the equation $\Delta_{M^n} = \Delta_{M_1} +\dots + \Delta_{M_n}$.
    \end{lemma}
    
\begin{proof}
    See Appendix \ref{sec: appendix a}.
\end{proof}
  
We have the following preliminary result.
    \begin{lemma}\label{lemma: Brownian motion on product manifold}
        Suppose $X^1, \dots, X^n$ are independent Brownian motions on $M$. Then each $X^j$ is a solution to
            \begin{align}
                dU_{t,j} & = H_i(U^j_t) \circ dW^i_{t,j},
                \\
                dX^k_t &= U_{t,k}(e_i) \circ dW^i_{t,k},
            \end{align}
        where $W_{t,k}^i$ are independent one-dimensional real-valued Brownian motion for $0 \leq i \leq d$ and $0 \leq j \leq n$. In particular, $X= (X^1,\dots, X^n)$ is a Brownian motion on $M^n$.
    \end{lemma}

\begin{proof}
    See Appendix \ref{sec: appendix a}.
\end{proof}
    

Let $c \colon \R_+ \times M^n \rightarrow \R$ be a $C^{1,2}$-function, then we have the following version of Girsanov's theorem.

\begin{theorem}\label{result: girsanov on product manifold}
Let $X$ be a Brownian motion on $M^n$ under $\Pb$. Assume that $X$ is non-explosive, e.g., $M^n$ a compact manifold. For any measurable vector field $c_t$ on $M$ satisfying, for $T > 0$,  $\int_0^T \lVert c(s,X_s)\rVert^2 ds < \infty $, $\Pb$-a.s.., and $c = c_1 \oplus \cdots \oplus c_n$, we can define a measure $\Pb^c_t$ on $\cF_t$, for $t\in[0,T]$, by 
    \begin{equation}
        \frac{d\Pb^c}{d\Pb}\bigg|_{\cF_t} (X) = \prod_{k=1}^n\exp\left\{  \int_0^t \left\langle c_k(s,X_s), dX^k\right\rangle_{g_k} - \frac{1}{2}\int_0^t \lVert c_k(s,X_s)\rVert^2_{g_k} ds \right\}.
    \end{equation}
\end{theorem}

\begin{proof}
From \cite[Chapter 4, Proposition 1B]{elworthy1988geometric} it follows that 
    \begin{equation*}
        \frac{d\Pb^c}{d\Pb}\bigg|_{\cF_t} (X) = \exp\left\{  \int_0^t \left\langle c(s,X_s), U_sdW_s\right\rangle_g - \frac{1}{2}\int_0^t \lVert c(s,X_s)\rVert^2_g ds \right\},
    \end{equation*}
where $U$ is a horizontal Brownian motion on $O(M^n)$ solution to $dU_t = H_i(U_t) \circ dW^i_t$, for $1\leq i \leq nd$. From \reflemma{lemma: Brownian motion on product manifold} and that $g$ is a diagonal block matrix with diagonal elements $g_1,\dots, g_k$ the conclusion follows.
\end{proof}

As a first application of \refthm{result: girsanov on product manifold}, let once again $X_1,\dots, X_n$ be independent Brownian motions on $M$ with corresponding transition densities $p^1,\dots, p^n$. Then $X=(X^1,\dots,X_n)$ is a Brownian motion on $M^n$ with transition density $\rho_t(x,y) = \prod_{i=1}^n p^i_t(x_i,y_i)$, for every $x,y \in M^n$. The vector field $\nabla_x \log \rho_t(x,v)$ on $M^n$ satisfies the assumptions in \refthm{result: girsanov on product manifold}. We can define the Radon-Nikodym derivative by
    \begin{equation*}
        \frac{d\Pb^\rho}{d\Pb_x}\bigg|_{\cF_t} (X)  = \frac{\rho_{T-t}(X_t, v)}{\rho_T(x,v)}.
    \end{equation*}
The Radon-Nikodym is seen to be a positive local-martingale under $\Pb_x$ on $[0,T)$ with initial value of one. By \refthm{result: girsanov on product manifold}, the Radon-Nikodym can be expressed as
    \begin{equation}
        \frac{d\Pb^\rho}{d\Pb_x}\bigg|_{\cF_t} (X) = \prod_{k=1}^n e^{  \int_0^t \left\langle \nabla_{X_t} \log p^k_{T-t}(X_T,v_i), dX^k\right\rangle_{g_k} - \frac{1}{2}\int_0^t \lVert \nabla_{X_t} \log p^k_{T-t}(X_t,v_i),\rVert^2_{g_k} ds},
    \end{equation}
which is exactly the product of the law of $n$ Brownian bridges on $M$, conditioned on $v_1,\dots,v_n$ at time $T>0$, respectively.


Let $U$ be a horizontal Brownian motion on the frame bundle $O(M^n)$, i.e., $U$ is a solution to the SDE
    \begin{equation}
        dU_t = H_k(U_t) \circ dW^k_t \quad \text{for} \quad 1 \leq k \leq nd,
    \end{equation}
where $W$ is an $\R^{nd}$ standard Brownian motion. Let $h$ be a vector field on $M^n$ of the form $h = h_1 \oplus \cdots \oplus h_n$ and let $g$, the Riemannian metric on $M^n$ be a block diagonal matrix with diagonal elements $g_1,\dots, g_n$, where $g_j$ denotes the Riemannian metric on $M_j$ (the $j$'th component in the product manifold). We then have
    \begin{align*}
        \frac{d\Pb^h}{d\Pb}\bigg|_{\cF_t} (X)
        &
        = e^{\int_0^t \left\langle h(s,X_s), U(e_k)\right\rangle dW^k_t - \frac{1}{2} \int_0^t h^T(s,X_s) g(X_s) h(s,X_s) ds} 
        \\
         &
        = \prod_{i=1}^n e^{\int_0^t \left\langle h_1(s,X_s), U(e_k)\right\rangle dW^k_t - \frac{1}{2} \int_0^t h^T_i(s,X_s) g_i(X_s) h_i(s,X_s) ds}.
    \end{align*}
The latter equation is seen to equal the product law $\prod_{i=1}^n \frac{d\Pb^{h_i}}{d\Pb}\big|_{\cF_t} (X)$.



\fi




\input{Content/Sub-content/Conditioning_on_submanifold}


    
\subsection{Numerical Schemes}

In this section, we present two numerical schemes for estimating the weighted diffusion mean by sampling Brownian bridges on $M^n$ conditioned on hitting the diagonal $N= \diag(M^n)$:
    \begin{enumerate}
        \item The first method is based Marchand \cite{marchand2011conditioning}. Focusing on a single chart representation of the manifold, a similar type of conditioning as presented by Marchand is obtained. Using a suitable transformation $L$, whose kernel is the diagonal $\diag(M^n)$, results in the guided bridge process converging to the diagonal. An explicit expression for the likehood is given. Moreover, we argue that the single chart representation is not a limitation since connected manifolds can be covered by a single chart up to a set of measure zero. Introducing a sequence of stopping times, the process can be regarded in the above local sense on each stochastic interval.
        
        \item The second method is based on the paper by Delyon and Hu \cite{delyon_simulation_2006}. Using local coordinate charts, the weighted arithmetic mean $\mu(x) = \frac{\sum_i w_i x^i}{\sum_j w_j}$ can be calculated locally and used as a pinning point. Centering each new coordinate chart around $\mu(x)$, leads to convergence of the guided process to the diagonal. Moreover, an explicit expression for the likelihood is obtained similar to that of \cite[Theorem 6]{delyon_simulation_2006}.
    \end{enumerate}
    
%Embedding the product manifold in $\R^N$, the extrinsic mean on the diagonal acts as the conditioning point in each iteration.
%    \begin{remark}
%        There are infinitely many ways to embed a manifold in $\R^N$. This is the primary aversion against using extrinsic means over intrinsic ones like the Fréchet-mean. 
%    \end{remark}
%    
%Figure \ref{fig: bridges conditioned on average} illustrate the second method using coordinate charts of $\mathbb S^2$. In particular, the figure show a situation where the diffusion sample mean better predicts the true mean value. It should however be noted, that a different sample of the guided process may lead to another sample estimate.
    
%For each parameterization $\{(D_{\alpha}, \phi_{\alpha})\}_{\alpha}$ of $M$ there exists an increasing sequence of predictable stopping times $0 \leq T_k \leq T_{k+1}$ such that on each stochastic interval $\llbracket T_k, T_{k+1}\rrbracket = \{(\omega,t)\in \Omega \times \R_+| T_k(\omega) \leq t \leq T_{k+1}(\omega)\}$ the process $x_t \in D_{\alpha}$, for some $\alpha$ (see \cite[Lemma 3.5]{emery1989stochastic}). Thus, the Brownian motion $x$ on $M$ can be described locally in a chart $D_{\alpha} \subset M$ as the solution to the system of SDEs, for $(\omega,t) \in \llbracket T_k, T_{k+1} \rrbracket \cap \{T_k < T_{k+1}\}$
%    \begin{equation}\label{eq: local brownian motion}
%        dx_t^i(\omega) = b^i(x_t(\omega))dt + \sigma^i_j(x_t(\omega)) dW^j_t(\omega), 
%    \end{equation}
%where $\sigma$ denotes the matrix square root of the inverse of the Riemannian metric tensor $(g^{ij})$ and $b^k(x) = - \frac{1}{2}g^{ij}(x)\Gamma^k_{ij}(x)$ is the contraction over the Christoffel symbols (see, e.g., \cite[Chapter 3]{hsu2002stochastic}). Strictly speaking, the solution of equation \eqref{eq: local brownian motion} is defined by $x_t^i = \phi_{\alpha}(x_t)^i$. 

We will need the following version of Girsanov's theorem that uses the coordinate representation of the Browniation motion \eqref{eq: local brownian motion}.
%Recall that (see e.g., \cite{hsu2002stochastic})
%    \begin{equation}
%        dx_t = b(x_t)dt + \sigma(x_t)dW_t,
%    \end{equation}
%is a Brownian motion on $M$ written in local coordinates. In particular, if $X_t$ is a Brownian motion on $M$ and $\left(U_{\alpha},\phi_{\alpha}\right)$ a countable open covering of $M$, then there exists a sequence of non-decreasing predictable stopping times $T_k$ such that on each stochastic interval $\llbracket T_k, T_{k+1}\rrbracket$ the process $X$ takes its values in one of the $U_{\alpha}$'s. Then $X$ can be expressed as
%    \begin{equation}
%        1_{\llbracket T_k, T_{k+1}\rrbracket}dX_t = b_k(X_t)dt + \sigma_k(X_t)dW_t, \quad X_0 = x.
%    \end{equation}

    \begin{theorem}
        Let $X$ be a Brownian motion on $M$ such that on each interval $\llbracket T_k, T_{k+1}\rrbracket$, $X$ takes its values in some open set $U_{\alpha}$. Define $Z$ as the solution to 
            \begin{equation}
                dZ_t = \sigma_k(Z_t)dW_t, \quad Z_{T_k} = X_{T_k},
            \end{equation}
        and let $\tilde T_{k+1}$ be the predictable stopping where $Z$ exits $U_{\alpha}$. Then 
            \begin{equation}
                \E\left[f(X)\right] = \E\left[f(Z)e^{\int_{T_k}^{T_{k+1}\wedge \tilde T_{k+1}} b^T_k(Z_t)A(Z_t) dZ_t - \frac{1}{2}\int_{T_k}^{T_{k+1}\wedge \tilde T_{k+1}} \lVert \sigma_k^{-1}(Z_t)b_k(Z_t)\rVert^2 dt} \right].
            \end{equation}
    \end{theorem}
    
    \begin{proof}
        On the interval $\llbracket T_k , T_{k+1}\wedge \tilde T_{k+1} \rrbracket$, both process are Euclidean valued and thus the result follows from the usual Girsanov's theorem.
    \end{proof}
    
 We make the following assumptions throughout.

\begin{assumption}\label{assumption: 2 in delyon and hu}
In every chart, the square root of the cometric tensor, denoted by $\sigma$, is $C^2$. Furthermore, $\sigma$ and its derivatives are bounded; $\sigma$ is invertible with bounded inverse. The drift $b$ is locally Lipschitz and locally bounded.
\end{assumption}



\subsubsection{Scheme 1}


We here first assume that $M$ can be covered by a single chart. %and that the Ricci curvature of $M$ is bounded below. This later condition ensures the long term existence of a Brownian motion on $M$ and hence that $M$ is stochastically complete, i.e., $\int_M p_t(x,y) d\Vol_M(y) = 1$, for all $t \geq 0$ and all $x \in M$.
%Let $dx_t = b(x_t)dt + \sigma(x_t)dW_t$ be the vector valued version of equation \eqref{eq: local brownian motion}. 
Let $x_1, \dots, x_n \in M$ be observations and let $X_{t,1}, \dots, X_{t,n}$ be independent Brownian motions with $X_{0,1}=x_1,\dots, X_{0,n}=x_n$. Using the coordinate SDE \eqref{eq: local brownian motion} for each $X_{i,t}$, we can write the entire system on $M^n$ as
%the observations together, we obtain a tuple $(x_1,\dots,x_n) \in M^n$ and the system of equations $dX_{t,1},\dots,X_{t,n}$ can be written in differential form as a solution on $M^n$ of the SDE
\begin{equation}\label{eq: local brownian motion on product manifold}
    d
    \begin{pmatrix}
        X^1_{t,1} \\ 
        \vdots \\ 
        X^1_{t,n}\\
        \vdots \\
        X^d_{t,1} \\
        \vdots \\
        X^d_{t,n}
    \end{pmatrix}
        =
        \begin{pmatrix}
            b^1(X_{t,1}) \\ 
            \vdots \\ 
            b^1(X_{t,n})\\
            \vdots \\
            b^d(X_{t,1}) \\ 
            \vdots \\
            b^d(X_{t,n})
        \end{pmatrix}
        dt
        +
        \left[\begin{array}{ccc}
\Sigma_{1}(X_{t,1},\dots,X_{t,n}) \\
\vdots   \\
\Sigma_d(X_{t,1},\dots,X_{t,n}) \\
\end{array}\right] d W_t,
\end{equation}
where $\Sigma_j$ is an $nd \times nd$ diagonal matrix with each diagonal element the row vector $\sigma_{j\cdot}(X_{t,i})$, and $W$ is the column vector $(W_{t,1}^T \dots W_{t,n}^T)^T$. By \refass{assumption: 2 in delyon and hu}, the diffusion coefficient above, denoted $\Sigma$, is $C^2$, invertible, and $\Sigma$, its inverse and its derivatives are bounded. Moreover, the drift coefficient, denoted $\tilde b$, is locally Lipschitz and locally bounded. 

Denote the solution to \eqref{eq: local brownian motion on product manifold} by $X_t$, then we can write \eqref{eq: local brownian motion on product manifold} more compactly as
\begin{equation}
    dX_t = \tilde b(X_t)dt + \Sigma(X_t)d W_t.
\end{equation}
The conditioning $X_T\in N$ is equivalent to the requirement $X_{T,1}^k = \cdots = X_{T,n}^k$, for every $1 \leq k \leq d$ and, in coordinates, $X_t\in\diag(\mathbb R^{nd})$.
%ince $X^k_{T,j} \in \R$, for every $1\leq j \leq n$, the above conditioning is equivalent to the requirement $\{X^k_{T,j}\}_{j=1}^n$ resides in the diagonal $D \subseteq \R^n$, for each $1 \leq k \leq d$, 
We let $L\in M^{nd\times nd}$ be a matrix with orthonormal rows satisfying $\ker L = D^d := D \times \cdots \times D $ so that the desired conditioning reads $LX_T = 0$. The following lemma provides a sufficient condition on $L$ such that $\ker L = D^d$.
%
%\begin{lemma}
%    If $L$ is an $(n-1)d \times nd$ matrix of rank $(n-1)d$ whose rows sum to zero, then $\ker L = D^d$.
%\end{lemma}
%
%\begin{proof}
%    Without loss of generality, we may assume that $L$ is a diagonal matrix where each diagonal element in the matrix $L$ is a $(n-1)\times n$ matrix with rank $n-1$ whose rows are summing to zero. Then it suffices to show the result for the diagonal element. With slight abuse of notation, we denote the diagonal element by $L$ as well. 
%    
%    Let $x \in D$. The $i$'th component $(Lx)_i = 0$, for every $1 \leq i \leq n-1$, since $x = a(e_1+ \cdots + e_n)$, for a scalar value $a$, and the rows of $L$ sum to zero. Hence $x \in \ker L$. Since $D$ is isomorphic to $\R$, by the rank-nullity theorem, we conclude that $\ker L = D$.
%\end{proof}
Define the following oblique projection, similar to \cite{marchand2011conditioning} with $k=1$,
\begin{equation}
    P_t(z) = a(z)L^T A(z) L,
\end{equation}
where
    \begin{equation*}
        a(z) = \Sigma(z)\Sigma(z)^T \quad \text{and} \quad A_t(z) = (La(z)L^T)^{-1}.
    \end{equation*}
Moreover, set 
    \begin{equation*}
        \beta(z) = \Sigma(z)^T L^T A(z) \quad \text{and} \quad \eta(z) =  \sqrt{\det(A(z))}.
    \end{equation*}
With the above defined processes equation \eqref{eq: marchand sde} can be written as
    \begin{equation}\label{eq: marchand SDE on manifold}
        dY_t = \tilde b(Y_t)dt + \Sigma(Y_t)d\tilde W_t - \Sigma(Y_t)\beta(Y_t)  \frac{LY_t}{T-t} 1_{(T-\varepsilon,T)}(t)dt, \quad Y_0 = u.
    \end{equation}
    
We have the following result under the assumption that $\tilde b$ is locally Lipschitz and locally bounded.    
    
\begin{lemma}\label{result: convergence lemma marchand}
Equation \eqref{eq: marchand SDE on manifold} with random initial condition $u$ admits a unique solution on $[0,T)$. Moreover, $\lVert L Y_t \rVert^2 \leq C(\omega) (T-t) \log \log [(T-t)^{-1} + e]$ a.s., where $C$ is a positive random variable.
\end{lemma}

\begin{proof}
    Since $L P = L$, the proof is similar to the proof of  \cite[Lemma 6]{marchand2011conditioning}.
\end{proof}

    
With the same assumtions, we get as well the following result similar to \cite[Theorem 3]{marchand2011conditioning}.

\begin{theorem}
Assume that $\Sigma$ and $a^{-1}$ are $C^2_b$-functions. Let $Y_t$ be a solution of \eqref{eq: marchand SDE on manifold}, where $\tilde b$ is exchanged with $\hat b$ which is $C^2_b$-function. Then for any bounded function $f$ on $M$,
    \begin{equation}
        \E\left[f(X)|X_T \in L^{-1}(0)\right] 
        =
        C\E\left[f(y) \varphi(Y_T)\right], 
    \end{equation}
where $C$ is a positive constant, $\check b = \tilde b - \hat b$, and 
    \begin{align}
        \varphi(Y_t) 
        &
        =
        \eta(Y_T) \exp\bigg\{- \frac{\lVert \beta_{T-\varepsilon}(Y_{T-\varepsilon})LY_{T-\varepsilon}\rVert^2}{2\varepsilon} 
        \\
         -
         &
         \int_{T-\varepsilon}^T \frac{2(LY_s)^TL\hat b(Y_s)ds - (LY_s)^Td(A(Y_s)) LY_s + d[A(Y_s)^{ij}, (LY_s)_i(LY_s)_j]}{2(T-s)}
         \\
         &
         +
         \int_0^T \check b(Y_s)a(Y_s)^{-1}dY_s - \frac{1}{2}\lVert \Sigma(Y_s)^{-1}\check b(Y_s)\rVert^2ds
        \bigg\}
    \end{align}
\end{theorem}

\begin{proof}
    A direct consequence of \cite[Theorem 3]{marchand2011conditioning}, for $k=1$, and \reflemma{result: convergence lemma marchand}.
\end{proof}

Since connected manifolds can be covered by a single chart up to a set of measure zero (e.g. a geodesic chart up to the cut locus), we can consider an non-decreasing sequence of predictable stopping times such that on each stochastic interval, the process belongs to the chart. Consider the process $1_{\llbracket T_k, T_{k+1} \rrbracket} Y_t$, then on each $\llbracket T_k, T_{k+1} \rrbracket$ $Y_t$ can be written locally as in \eqref{eq: marchand SDE on manifold} and we have the following result.

\begin{lemma}
The process $Y$ converges in the following sense: $ 1_{\llbracket T_k, T_{k+1}\rrbracket}\lVert L_k Y_t \rVert^2 \leq C_k(\omega) (T-t) \log \log [(T-t)^{-1} + e]$ a.s., where $C_k$ is a positive random variable and where subscript $k$ intervals wherein the process stays in the chart.
\end{lemma}

\begin{proof}
    Follows from \reflemma{result: convergence lemma marchand} in each chart.
\end{proof}

\begin{theorem}
Assume that $\Sigma$ and $a^{-1}$ are $C^2_b$-functions. Let $Y_t$ be a solution of 
    \begin{equation}
        dY_t = \tilde b_k(Y_t)dt + \Sigma_k(Y_t)d\tilde W_t - \Sigma_k(Y_t)\beta_k(Y_t)  \frac{L_kY_t}{T-t} 1_{\llbracket T_k-\varepsilon_k,T_k \rrbracket}(t)dt, \quad Y_0 = u,
    \end{equation}
on each stochastic interval $\llbracket T_k, T_{k+1} \rrbracket$, where $\tilde b$ is exchanged with $\hat b$ which is $C^2_b$-function and the subscript $k$ denotes the chart dependence. Then for any bounded function $f$ on $M$,
    \begin{equation}
        \E\left[f(X)|X_T \in L^{-1}(0)\right] 
        =
        C\E\left[f(y) \varphi(Y_T)\right], 
    \end{equation}
where $C$ is a positive constant, $\check b = \tilde b - \hat b$, and 
    \begin{align}
        \varphi(Y_t) 
        &
        =
        \prod_{k=1}^\infty \eta(Y_{T_{k}})\exp\bigg\{- \frac{\lVert \beta_{T_k-\varepsilon_k}(Y_{T_k-\varepsilon_k})L_kY_{T_k-\varepsilon_k}\rVert^2}{2\varepsilon_k} 
        \\
         -
         &
         \int_{T_k-\varepsilon_k}^{T_k} \frac{2(L_kY_s)^TL_k\hat b_k(Y_s)ds - (L_kY_s)^Td(A_k(Y_s)) L_kY_s }{2(T-s)}
         \\
         +
         &
        \int_{T_k-\varepsilon_k}^{T_k} \frac{d[A_k(Y_s)^{ij}, (L_kY_s)_i(L_kY_s)_j]}{2(T-s)}
         \\
         &
         +
         \int_{T_k}^{T_{k+1}} \check b_k(Y_s)a_k(Y_s)^{-1}dY_s - \frac{1}{2}\lVert \Sigma_k(Y_s)^{-1}\check b_k(Y_s)\rVert^2ds
        \bigg\}
    \end{align}
\end{theorem}

\begin{proof}
    A direct consequence of \cite[Theorem 3]{marchand2011conditioning} for $k=1$.
\end{proof}




\subsubsection{Scheme 2}


We now consider the guiding term introduced by Delyon and Hu \cite{delyon_simulation_2006}. In particular, we will be conditioning on a functional of its path. Conditioning on linear functionals of its path was studied by Sottinen and Yazigi \cite{sottinen2014generalized}. Sottinen and Yazigi considered two representations: an orthogonal and a canonical. The orthogonal representation requires the knowledge of the future whereas the canonical representation does not. If the charts we consider was not centered around the weighted mean point, the canonical representation of \cite{sottinen2014generalized} could be applied and the likelihood could be evaluated using automatic differentiation.


Let $x_1,\dots, x_n$ be observations in $M$ and pick a chart $D$ sufficiently big such that $x_1,\dots,x_n \in D$ (this requirement can be loosened by only requiring some of the initial values be in $D$). Furthermore, let $X^1_t,\dots, X^n_t$ be Brownian motions each of which satisfying the system of equations in \eqref{eq: local brownian motion}, with $X^1_0 = x_1, \dots, X^n_0 = x_n$. In the coordinate chart, we can calculate a coordinate weighted average of the current positions of the Brownian motion as $\mu(x) = \frac{\sum_{i=1}^n w_i X^i_t}{\sum_{i=1}^n w_i}$. Similar to Sommer and Bronstein \cite{sommer2020horizontal}, we consider the case where a process $X_t$ is conditioned on $\mu(x)$.

Define $Y_t=(Y^1_t,\dots, Y^n_t)$ as the solution to the system of SDEs written in local coordinates, for $(\omega,t)\in  \llbracket T_k, T_{k+1} \rrbracket \cap \{T_k < T_{k+1}\}$,
    \begin{equation}\label{eq: guided process locally in chart}
        dy^i_t(\omega) = \left(b^i(y_t(\omega)) - \frac{y^i_t(\omega)-\mu^i(y_t(\omega))}{T-t}\right)dt  + \sigma^i_j(y_t(\omega))dW^j_{t,i}(\omega),
    \end{equation}
where $\mu(y_t) = \left(\frac{\sum_{i=1}^n w_i y^i_t}{\sum_{i=1}^n w_i}, \dots, \frac{\sum_{i=1}^n w_i y^i_t}{\sum_{i=1}^n w_i}\right)$. Assuming that $M$ can be covered by a single chart and that the conditions in \refass{assumption: 2 in delyon and hu} are satisfied, we have the following version of \cite[Lemma 4]{delyon_simulation_2006}.


    \begin{lemma}\label{result: local convergence}
        Suppose $M$ can be covered by a single chart. Under the \refass{assumption: 2 in delyon and hu}, the system of SDEs given by \eqref{eq: guided process locally in chart} converges almost surely to $\mu(Y_T)$.
    \end{lemma}
    
    \begin{proof}
                By \reflemma{result: delyon hu type lemma}, conditioning on a suitable transformation of a diffusion process leads to almost sure convergence. 
                Note that $\mu(t)$ always belongs to the interior of the convex hull spanned by the coordinate points $y^i_t$. In particular, any diffusion process with initial value belonging to the convex hull will do. Consequently, the desired conditioning and convergence then follows from this more general conditioning.
        
        
        
        
        \iffalse
        For the proof we will need the result in Appendix B. %\ref{sec: appendix b}  
        Let $z$ be the solution to the SDE defined on $[S,T)$ for some $S\in (0,T)$
            \begin{equation}
                dz_t = b(z_t)dt - \frac{z_t - v}{T-t}dt + \sigma(z_t) dB_t,
            \end{equation}
        for an $d$-dimensional Brownian motion $B$. Then $z$ converges a.s. by \cite[Lemma 4]{delyon_simulation_2006}. Next, consider the SDE
            \begin{equation}
                dy_t  = 1_{[0,S)}(t)\left(b(y_t)dt - \frac{y_t - z_t}{S-t}dt + \sigma(y_t) dW_t \right) + 1_{[S,T)} dz_t.
            \end{equation}
        By \reflemma{result: delyon hu type lemma}, the above SDE converges a.s. and it remains to let $S \uparrow T$.
        \fi
        
    \end{proof}
As a special case of the result above, assume the existence of a sequence of stopping times $(S_t)_k$ such that for
$(\omega,t)\in  \llbracket S_k,S_{k+1} \rrbracket \cap \{S_k < S_{k+1}\}$, the process $y$ defined locally by \eqref{eq: guided process locally in chart} belongs to the coordinate chart $U_k$ centered at $\mu(y_{S_k})$. Then on $\llbracket S_k, S_{k+1}\rrbracket$ $y$ also satisfies the local equation 
    \begin{equation}
        dy_t = \left(b_k(y_t) - \frac{y_t}{T-t}\right)dt  +  \prescript{}{k}{\sigma(y_t)}dW_{t},
    \end{equation}
where $b^k$ and $\prescript{}{k}{\sigma(y_t)}$ denote the chart depends of the coefficients.
From the preceding lemma, the process $y$ converges almost surely. In this restrictive setting we obtain the manifold equivalent of \cite[Theorem 6]{delyon_simulation_2006}.



\begin{theorem}\label{result: delyon hu thm 6}
Let $M$ be covered by a single chart and \refass{assumption: 2 in delyon and hu} hold. Let $y$ be the solution to 
    \begin{align}
        dy_t
        &
        =  - \frac{y_t-v(z_t)}{T-t}dt + \sigma(y_t)dW_t\\
        dz_t 
        &
        = b_k(z_t)dt- \frac{z_t}{T-t}dt + \prescript{}{k}{\sigma(y_t)}d\tilde W_t,\label{eq: guided help}
    \end{align}
where $v(z) = \phi(\phi_k^{-1}(z))$.
Let $(S_k)_k$ be a sequence of stopping times such that $S_0=0$, $\lim_{k\rightarrow \infty} S_k = T$, and on each stochastic interval $z$ belongs to the coordinate chart $U_k$ centered at $\mu(z_{S_k})$. 
Then $\lim_{t\uparrow T}y_t = v(z_T) = \mu(y_T)$ a.s. and
    \begin{align}\label{eq: delyon hu correction}
        \E\big[f(x)|x_T &= \mu(y_T)\big] \nonumber
        \\
        &
        =
        C  \E\bigg[f(y) \exp\bigg\{\hspace{-1.mm}-\hspace{-1mm}\int_0^T \frac{ \tilde y^T_t \left(dA(y_t)\right)  \tilde y_t+\sum d\left\langle A^{ij}(y),\tilde y^i  \tilde y^j\right\rangle_t}{T-t}
        \\
        &
        + \int_0^T \left(b^T A\right)(y_t)dy_t -\frac{1}{2}\int_0^T \lVert \sigma^{-1} b \rVert^2 (y_t) dt\bigg\}\bigg], \nonumber
    \end{align}
where $\tilde y_t = y_t - v(z_t)$, $A = \left(\sigma^{-1}\right)^T \sigma^{-1}$, and $\langle \cdot,\cdot \rangle$ denotes the quadratic variation.
\end{theorem}

\begin{proof}
    By \reflemma{result: local convergence} $z_t$ converges a.s. and by \reflemma{result: delyon hu type lemma}, $y_t \rightarrow v(z_T)$ a.s. as $t \uparrow T$. By similar reasoning as in Theorem 5 and 6 of \cite{delyon_simulation_2006} we conclude.
\end{proof}

\begin{example}
In the case where the local chart is the exponential normal chart, equation \eqref{eq: guided process locally in chart} can be written on the form
    \begin{equation}\label{eq: guided process locally on weighted average}
        dy^i_t(\omega) = \left(b^i(y_t(\omega)) + \frac{\Log_{y^i_t(\omega)}(\mu^i(t))}{T-t}\right)dt  + \sigma^i_j(y_t)dW^j_{t,i}(\omega),
    \end{equation}
where $\Log_{y^i}$ is the inverse exponential map centered at $y^i\in M$. 
\end{example}


\iffalse


By similar arguments to that of \cite{jensen2021simulation, thompson2018brownian} the correction factor corresponding to \eqref{eq: guided process locally on weighted average}, with geometric local time $L$ on $\Cut(N)$, is given by
    \begin{equation}
        \varphi_t(y) = \exp\left\{\int_0^t \frac{r_{\mu(s)}(y_s)}{T-s}\left(d\eta_s + dL_s\right) \right\},
    \end{equation}
where $r_{\mu(t)}(y_t) = d(y_t,\mu(t))$, $\eta_t = \frac{\partial}{\partial r_{\mu(t)}} \log \Theta_{\mu(t)}^{-\frac{1}{2}}dt$, and $\frac{\partial}{\partial r_{\mu(t)}}$ denote differentiation in the radial direction.


Note that, similar to \eqref{eq: fermi bridge}, equation \eqref{eq: guided process locally on weighted average} can be expressed as $Y_t = \pi(V_t)$, where $V_t$ is defined as the solution to the guided process in $OM^n$
    \begin{equation}\label{eq: guided OM process}
        dV_t =  H_i(V_t) \circ \left(dW^i_t - \frac{\nabla^H \tilde d(V_t,\mu(t))^2}{2(T-t)}dt\right),
    \end{equation}
where $\nabla^H \tilde f(u)= \{H_1 \tilde f(u), \dots, H_{nd} \tilde f(u) \}$ and $\tilde f(u) = f(\pi(u))$, for some $f \in C^{\infty}(M^n)$. The following result generalizes \reflemma{result: local convergence}.

\begin{lemma}
Assume the conditions in \refass{assumption: 2 in delyon and hu} are satisfied and that there exist constants $\nu \geq 1$ and $\lambda \geq 0$ such that $\frac{1}{2}\Delta_M r_N^2 \leq \nu + \lambda r_N^2$ on $D\backslash \Cut(N)$, where $D$ is a regular neighborhood of $M^n$. Then $Y_t$, given by \eqref{eq: guided OM process}, converges almost surely to $\mu(T)$.
\end{lemma}

\begin{proof}
    Let $\tau_t(N)$ denote a tubular neighborhood around $N$ such that $\tau_t(N) \rightarrow N$ as $t \uparrow T$. Consider the guided process 
    \begin{align}\label{eq: guided help}
        dV_t =  H_i(V_t) \circ \bigg(dW^i_t 
        &
        - 1_{\tau_t(N)^c}(\pi(V_t))\frac{\nabla^H \tilde d(V_t,N)^2}{2(T-t)}dt \nonumber \\
        &
        - 1_{\tau_t(N)}(\pi(V_t))\frac{\nabla^H \tilde d(V_t,\mu(t))^2}{2(T-t)}dt
        \bigg),
    \end{align}
    where $\tau_t(N)^c = M^n \backslash \tau_t(N)$. Let $\tau_D$ denote the first exit time by $Y$ of $D$. From \cite[Theorem 2]{thompson2018brownian} 
    \begin{equation}\label{eq: james bound}
        \E\left[1_{\{t < \tau_D \}} r_N(Y_t)\right] \leq \left(\left(r_N(y_0)^2\left(\frac{T-t}{T}\right) + \nu t\right)\left(\frac{T-t}{T}\right)\right)^{1/2}e^{\lambda t/2},
    \end{equation}
where $Y_0=y_0$. Letting $(D_i)$ be an exhaustion of $M^n$ by regular neighborhoods, as $t \uparrow T$ and $i\uparrow \infty$ it follows that $Y_t$ belongs to a tubular neighborhood of $N$ (one can simply pick the radius of the tubular neighborhood as the right hand side of \eqref{eq: james bound}. From \reflemma{result: local convergence} the process converges a.s. on $[t_0,T)$, for $t_0$ large enough. What remains is to note that on $[0,T)$ the law of \eqref{eq: guided OM process} and \eqref{eq: guided help} are equivalent.
\end{proof}
    
\begin{example}
Parameterizing $M$ using an exponential normal chart, we obtain a coordinate chart which covers $M$ except for a subset of Riemannian volume measure zero. Working with the manifold $\tilde M := \exp_p(M)$ instead of $M$, we obtain a manifold with a pole at $p$. The same argument can be applied to product manifolds $M^d$. 
\end{example}

\fi

\section{Simulation on M}

In this section, we present algorithms for sampling the diffusion bridges on product manifolds. The sampling importance resampling (SIR) algorithm described in Algorithm~\ref{alg: weighted diffusion mean} yields an approximation of the weighted diffusion mean. For each sample $y^i$ of the guided bridge process, we compute the corresponding correction factor $\varphi_T(y_i)$. The resampling step then consists in picking $y_T^j$ with a probability determined by the correction terms, i.e., with $J$ number of samples we pick sample $j$ with probability $P_j = \frac{\varphi_T(y^j)}{\sum_{i=1}^J \varphi_T(y^i)}$. Algorithm~\ref{alg: bridge sampling on product manifold} simulates the process from \refthm{result: delyon hu thm 6}. We use the Euler-Maruyama discretization scheme. In each iteration, an auxiliary process is simulated locally in a chart centered at the weighted mean value in the chart $\mu(y_{t_k})$. This way, the pinning point of the auxiliary process is the origin of the chart. Mapping the point back to the original chart gives the pinning point for our guided process. Fig.~\ref{fig: Mean on sphere} illustrate an example of Algorithm~\ref{alg: bridge sampling on product manifold}.


\begin{algorithm} \DontPrintSemicolon \SetAlgoLined
\textbf{Input:} Points $x_1,\dots, x_n \in M$
\textbf{Output:} weighted Diffusion-Mean\\
\For{$j=1$ to $J$}{
Sample path from guided process $Y_t$\\
Record $Y_T^j$ and compute correction factor $\varphi_j(Y_T^j)$
}
Sample $j$ from $1,\dots, J$ with probability $P_j = \frac{\varphi_j(Y_T^j)}{\sum_{k=1}^J \varphi_k(Y_T^k)}$.\\
\tcp{Return $Y_T^j$}
\caption{weighted Diffusion Mean}
\label{alg: weighted diffusion mean}
\end{algorithm}
    



\begin{algorithm} \DontPrintSemicolon \SetAlgoLined
\caption{Bridge Sampling on Product Manifold}
\label{alg: bridge sampling on product manifold}
\textbf{Input:} $x_1,\dots, x_n \in M$ \;
\textbf{Output:} Bridge Sampling in $M^n$  \; 
\tcp{Initiate} The coordinate chart $D$ covers $M$ and weights $w_1,\dots w_n >0 $ \;
Define weighted average in $D$ as  
$\bar y_0= \frac{\sum_{j=1}^n w_j\phi(x_j)1_D(x_j)}{\sum_{k=1}^n w_k}$ \;
$y_{t_0} = (x_1,\dots,x_n)$ \;
In each time step \;
    \For{k = 1 to N}
{
    \tcp{Sample bridge step} 
    $z_{t_k} = z_{t_{k-1}} + \left(b_k(z_{t_{k-1}})-\frac{z_{t_{k-1}}}{T-t_{k-1}}\right) \Delta t + \prescript{}{_k}{\sigma(z_{t_{k-1}})} \Delta \tilde B_{t_{k-1}}$  \;
    $y_{t_k} = y_{t_{k-1}} + \sigma(y_{t_{k-1}}) \Delta B_{t_{k-1}}$ \;
    $y_{t_k} = y_{t_k} - \frac{y_{t_{k-1}} - v(z_{t_{k-1}})}{T-t_{k-1}} \Delta t$ \;
    \tcp{Compute the correction factor}
    $\log \varphi_{t_k} = \log \varphi_{t_{k-1}}- \tilde y_{t_{k}}^T\left(A(t_k,y_{t_k})-A(t_{k-1},y_{t_{k-1}})\right) \tilde y_{t_{k}}\frac{1}{2(T-t_k)} + (*)$  \;
    $(*)$ here denotes the last two terms of the correction term in \refthm{result: delyon hu thm 6} \;
    \tcp{Calculate weighted average} \
    $\bar y_k = \frac{\sum_{j=1}^n w_j \phi(y^j_{t_k})1_D(y^j_{t_k})}{\sum_{k=1}^n w_k}$
     \;
\tcp{Update coordinate chart $D_k$ of $M$ centered at $\bar y_k$} 
}
\end{algorithm}






==> Content/Introduction.tex <==
\section{Introduction}

%Sommer and Bronstein introduced two new concepts in geometric deep learning \cite{sommer2020horizontal}. Firstly, the authors proposed a novel method for constructing convolutions on Riemannian manifolds using stochastic horizontal flows in the frame bundle geometry. The method considers the curvature (holonomy) of the manifold, providing a method for transporting orientations in a continuous way. Secondly, the authors proposed a method for efficiently evaluating the manifold convolution layers based on sampling manifold-valued processes centered around a weighted diffusion mean. 
%In this paper, we investigate further the ideas put forward in the latter method.

The Euclidean expected value can be generalized to geometric spaces in several ways. Fréchet \cite{frechet1948elements} generalized the notion of mean values to arbitrary metric spaces as minimizers of the sum of squared distances. Fréchet's notion of mean values naturally includes Riemannian manifolds with a given metric structure. On manifolds without a given metric, for example, affine connection spaces, a notion of the mean can be defined as an exponential barycenter, see e.g. \cite{arnaudon2005barycenters,pennec_barycentric_2018}. Recently, Hansen et al. \cite{hansen2021diffusion, hansen2021diffusiongeometric} introduced a probabilistic notion of a mean, namely the diffusion mean. The diffusion-mean is defined as the most likely starting point of Brownian motion given the observed data. Varadhan's asymptotic formula relating the heat kernel with the Riemannian distance relates the diffusion mean and the Fréchet mean.
 
Computing sample estimators of geometric means is often in practice difficult. For example, estimating the Fréchet mean often requires evaluating the distance to each sample point at each step of an iterative optimization to find the optimal value. When closed-form solutions of geodesics are not available, the distances are themselves evaluated by minimizing over curves ending at the data points, thus leading to a nested optimization problem. This is generally a challenge in geometric statistics, the statistical analysis of geometric data. However, it can pose an even greater challenge in geometric deep learning, where a weighted version of the Fréchet mean is used to define a generalization of the Euclidean convolution taking values in a manifold \cite{chakraborty2018manifoldnet}. As the mean appears in each layer of the network, closed-form geodesics is in practice required for its evaluation to be sufficiently efficient. 

As an alternative to the weighted Fre\'echer mean, \cite{sommer2020horizontal} introduced a corresponding weighted version of the diffusion mean. 
Estimating the diffusion mean usually requires ability to evaluate the heat kernel making it often similarly computational difficult to estimate. However, \cite{sommer2020horizontal} also sketched a simulation based approach for estimating the (weighted) diffusion mean that avoids numerical optimization and estimation of the heat kernel. Here, a mean candidate is generated by simulating a single forward pass of a Brownian motion on a product manifold conditioned to hit the diagonal of the product space. The idea is sketched for samples in $\mathbb R^2$ in Figure~\ref{fig: projection and bridges onto diagonal}.

In this paper, we present a comprehensive investigation of this idea. In particular, we provide the necessary theoretical background and results for the construction, we present two seperate simulation schemes, and we demonstrate how the scheme can be implemented computationally on high-dimensional manifolds.
The bridge simulation scheme can be applied in any context where fast computation of a sample mean is required, e.g., in the contexts of CNN.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{.485\textwidth}
        \centering
        \def\svgwidth{0.95\textwidth}
        \input{mean_on_diagonal_.eps_tex}
        \caption{The mean estimator viewed as a projection onto the diagonal of a product manifold. Given a set $x_1,\dots, x_n \in M$, the tuple $(x_1,\dots, x_n)$ (blue dot) belongs to the product manifold $M\times \cdots \times M$. The mean estimator $\hat \mu$ can be identified with the projection of $(x_1,\dots,x_n)$ onto the diagonal $N$ (red dot).}\label{fig: projection onto diagonal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.485\textwidth}
        \centering
        % \includegraphics[width=0.95\linewidth]{Figures/2-dim_bridges_on_average_1png.pdf}
        \includegraphics[width=0.95\linewidth]{Figures/faezeh.pdf}
        \caption{Diffusion-mean estimator in $\R^2$ using Brownian bridges conditioned on the diagonal. Here a Brownian bridge $X_t = (X^1_t,\dots, X^4_t)$ in $\R^8$ conditioned on the diagonal $N \subseteq \R^8$, where each $X^j$ is a two-dimensional process. }\label{fig: bridges conditioned on average}
    \end{subfigure}
    \caption{Mean estimation using projection onto a subset. (Left) General idea behind conditioning on the diagonal of a product manifold. (Right) A bridge process on the product manifold $\R^{2\times4}$ conditioned on the diagonal. Here each coordinate process is visualized in $\R^2$.}\label{fig: projection and bridges onto diagonal}
\end{figure}





\subsection{Contribution}
We present a diffusion bridge simulation scheme on product manifolds conditioned on the diagonal. The simulation scheme, which is based on the idea of Sommer and Bronstein \cite{sommer2020horizontal}, yields estimates of the diffusion mean. We present three methods for simulating guided diffusions conditioned on the diagonal of a product manifold. The first method is a conceptual one connecting the ideas of Thompson \cite{thompson2015submanifold,thompson2018brownian} with pinning on the diagonal. The the latter two methods are of practical value.
We use the coordinate expression of a Brownian motion in charts to use the method presented by Marchand \cite{marchand2011conditioning} and Delyon \& Hu \cite{delyon_simulation_2006} for simulation of conditioned diffusion processes. We show how this provides a conditioning on the diagonal with explicit correction terms. 



\iffalse
\begin{figure}[ht]
        \centering
        % \includegraphics[width=0.95\linewidth]{Figures/2-dim_bridges_on_average_1png.pdf}
        \includegraphics[width=0.25\linewidth]{Figures/faezeh.pdf}
        \caption{Diffusion-mean estimator in $\R^2$ using Brownian bridges conditioned on the diagonal. Here a Brownian bridge $X_t = (X^1_t,\dots, X^4_t)$ in $\R^8$ conditioned on the diagonal $N \subseteq \R^8$, where each $X^j$ is a two-dimensional process. }\label{fig: bridges conditioned on average}
\end{figure}
\fi


\iffalse
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{.485\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{Figures/mean_on_diagonal_final.pdf}
        \caption{The mean estimator viewed as a projection onto the diagonal of a product manifold. Given a set $x_1,\dots, x_n \in M$, the tuple $(x_1,\dots, x_n)$ (blue dot) belongs to the product manifold $M\times \cdots \times M$. The mean estimator $\hat \mu$ can be identified with the projection of $(x_1,\dots,x_n)$ onto the diagonal $N$ (red dot).}\label{fig: projection onto diagonal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.485\textwidth}
        \centering
        % \includegraphics[width=0.95\linewidth]{Figures/2-dim_bridges_on_average_1png.pdf}
        \includegraphics[width=0.95\linewidth]{Figures/faezeh.pdf}
        \caption{Diffusion-mean estimator in $\R^2$ using Brownian bridges conditioned on the diagonal. Here a Brownian bridge $X_t = (X^1_t,\dots, X^4_t)$ in $\R^8$ conditioned on the diagonal $N \subseteq \R^8$, where each $X^j$ is a two-dimensional process. }\label{fig: bridges conditioned on average}
    \end{subfigure}
    \caption{Mean estimation using projection onto a subset. (Left) General idea behind conditioning on the diagonal of a product manifold. (Right) A bridge process on the product manifold $\R^{2\times4}$ conditioned on the diagonal. Here each coordinate process is visualized in $\R^2$.}\label{fig: projection and bridges onto diagonal}
\end{figure}

\fi

==> Content/Sub-content/Conditioning_on_submanifold.tex <==
%\subsection{Conditioning on Submanifolds}

%Consider a Brownian motion $X_t=(X_t^1, \dots X_t^n)$ in the product manifold $M^n$. With the requirement that $X_T^1 = \dots = X_T^n$, at some prespecified time $T> t \geq 0$, the conditioned process $X_t\big|X_T^1 = \dots = X_T^n$ essentially is equivalent to the conditioned process $X_t\big|\diag(M^n)$, where the diagonal of $M^n$ is defined by $\diag(M^n):=\{(x_1,\dots,x_n) \in M^n \colon x_1=\dots =x_n\}$. The diagonal $\diag(M^n)$ is a submanifold of $M^n$ which can be identified with $M$, i.e. $\diag(M^n) \simeq M$. 
Consider a Brownian motion $X_t=(X_t^1, \dots X_t^n)$ in the product manifold $M^n$ conditioned on $X_T^1 = \dots = X_T^n$ or, equivalently, $X_T\in\diag(M^n)$. 
Since $\diag(M^n)$ is a submanifold of $M^n$, the conditioned diffusion defined above is absolutely continuous with respect to the Fermi bridge on $[0,T)$ \cite{thompson2015submanifold, thompson2018brownian}. To shorten notation, set $N=\diag(M^n)$ and define the horizontal guided process
    \begin{equation}\label{eq: fermi bridge}
        dU_t = H_i(U_t) \circ \left(dW^i_t - \frac{H_i \tilde r_N^2(U_t) }{2(T-t)}dt \right),
    \end{equation}
where $\tilde r$ denotes the lift of the radial process defined by $\tilde r_N(u) := r_N(\pi(u))= d(\pi(u), N)$. Here the distance to $N$ is $d(x,N):= \inf \{d(x,z) | z\in N\}$. The nominator in the drift term in \eqref{eq: fermi bridge} is the gradient of the squared distance to the diagonal and thus can be written as the i'th component of the Riemannian logarithm map, i.e., $(H_i \tilde r_N^2(U_t) = \log_{\pi(U_t)}(N))^i$. The Fermi bridge $Y$ is the projection of $U$ to $M$, i.e., $Y_t := \pi(U_t)$. We immediately have the following result.

\begin{theorem}
    For all continuous bounded functions $f$ on $M^n$, we have
        \begin{equation}
            \E^\Pb\left[f(X)|X_{T,1} = \cdots = X_{T,n}\right] =  \lim_{t \uparrow T}C\E^\Qb\left[f(Y)\varphi(Y_t)\right], 
            \label{eq:diagthm}
        \end{equation}
    for some positive constant $C$, where 
       \begin{equation*}
			d\log \varphi_t = 
	\frac{r_N(Y_t)}{T-t} \left(d\eta_s + dL_s\right) \quad \text{with} \quad 	d\eta_s = \frac{\partial}{\partial r_N} \log \Theta_N^{-\frac{1}{2}}ds,
		\end{equation*}
    and $L$ the geometric local time on $\Cut(N)$.
    \label{thm:diag}
\end{theorem}

\begin{proof}
From \cite[Theorem 8]{jensen2021simulation} and \cite{thompson2018brownian}, we have 
    \begin{equation*}
        \E^\Pb\left[f(X)|X_T \in N\right] = \lim_{t \uparrow T}C\E^\Qb\left[f(Y)\varphi(Y_t)\right].
    \end{equation*}
By definition of $N$, $X_T \in N$ if and only if $X_{T,1} = \cdots = X_{T,n}$.
\end{proof}
The result can be extended to the entire interval $[0,T]$ under certain conditions:
\begin{corollary}\label{result: james corollary}
    If $\Cut(N)$ is polar for $Y$, (i.e., the first hitting time of $\Cut(N)$ by $Y$ is a.s. infinite) and if either of the following conditions are satisfied
    \begin{itemize}
        \item[i)] the sectional curvature of planes containing the radial direction is 
            \begin{itemize}
                \item[1.] Non-positive
                \item[2.] Non-negative
            \end{itemize}
        \item[iii)] the Ricci-curvature in the radial direction is
            \begin{itemize}
                \item[1.] Non-positive
                \item[2.] Non-negative
            \end{itemize}
    \end{itemize}
then
    \begin{equation*}
        \E^\Pb\left[f(X)|X_{T,1} = \cdots = X_{T,n}\right] =  C\E^\Qb\left[f(Y)\varphi(Y_T)\right].
    \end{equation*}
In particular, $\frac{\varphi_T}{\E^\Qb[\varphi_T]} d\Qb \propto d\Pb_{|X_{T,1}=\cdots =  X_{T,n}}$.
\end{corollary} 

\begin{proof}
    Since $N$ is a totally geodesic submanifold of dimension $d$, the result follows from \cite[Appendix C]{thompson2015submanifold}.
\end{proof}

The conditions in \refcor{result: james corollary} quite restrictive. For example, consider the $2$-torus $\T^2 = \mathbb S^1 \times \mathbb S^1$. The diagonal $N$ is the curve in $\T^2$ rotating one round in both the toroidal and poloidal direction. The cut locus of $N$ is a similar curve in $\T^2$ corresponding to the antipodal points in $\mathbb S^1$. For $T>0$ large, the condition that $\Cut(N)$ is polar for $Y$ will not be satisfied. And certainly not if $Y_0= y \in \Cut(N)$. However, for numerical purposes, the equivalence \eqref{eq:diagthm} in Theorem~\ref{thm:diag} is sufficient as the interval $[0,T]$ is anyway finitely discretized.

\iffalse
Parameterizing $M$ using coordinate charts, the SDE for \eqref{eq: fermi bridge} in $M$ can be expressed in local coordinates by
\begin{equation}\label{eq: guided process in chart}
    dY_t = \left(b(Y_t) +  \frac{\Log_{Y_t}(N)}{T-t}\right)dt + \sigma(Y_t) dW_t,
\end{equation}
where $Y_t := \pi(U_t)$, $\sigma$ denotes the matrix square root of the inverse of the Riemannian metric tensor, $b(z)^k = - \frac{1}{2}g^{ij}(x)\Gamma^k_{ij}(z)$ is the contraction over the Christoffel symbols, and $\Log_z(N) := \inf_{p \in N} \Log_z(p)$. 
\fi




==> Content/Sub-content/Euclidean_example.tex <==
\subsection{Euclidean Case}

As a motivating example, we consider the case where $M = \R^d$. Let $\hat Y_t$ denote the time $t$-sample average $\tfrac{1}{n} \sum_{i=1}^n Y_t^i$, where the $(Y^i)'s$ are solutions to the system of equations
    \begin{align}
        dY^1_t 
        =
        &
        - \frac{Y^1_t - \hat Y_t}{T-t}dt + \sigma(Y^1_t) dW_t^1 \nonumber
        \\
        \vdots
        \\
        dY_t^n
        =
        &
        - \frac{Y^n_t - \hat Y_t}{T-t}dt + \sigma(Y^n_t) dW_t^n. \nonumber
    \end{align}
Under suitable regularity conditions, the system of equations converge to the arithmetic mean $\hat Y_T$ (CHECK THIS). Letting $Y_t = (Y^1_t,\dots, Y^n_t)$, we obtain a process in $\R^{d\times n}$ conditioned on the diagonal in $\R^{d\times n}$. We can write the system of equations more compactly as
    \begin{equation}
        dY_t = - A(t)Y_t dt + \Sigma dW_t,
    \end{equation}
where $A(t) = \frac{1}{T-t} A$ and $A$ is an $d \times d$ matrix with $1-1/n$ in the diagonal and $-1/n$ elsewhere, $\Sigma$ an $d \times d$ matrix with diagonal elements $\sigma_t(Y^i_t)$, and $dW_t$ the vectorized Brownian motion.


==> Content/Sub-content/bridges.tex <==
\subsection{Diffusion Bridges}

The sampling scheme for the (weighted) diffusion mean builds on simulation methods for conditioned diffusion processes, diffusion bridges. We here outline ways to simulate conditioned diffusion processes numerically in both the Euclidean and manifold context.

\subsubsection{Euclidean Diffusion Bridges}

Let $(\Omega, \cF, \cF_t, \Pb)$ be a filtered probability space, and $X$ a $d$-dimensional Euclidean diffusion solution on $[0,T]$ satisfying the stochastic differential equation (SDE) 
    \begin{equation}
        dX_t = b_t(X_t)dt + \sigma_t(X_t) dW_t, \quad X_0 = x,
    \end{equation}
where $W$ is a $d$-dimensional Brownian motion. Let $v\in\mathbb R^d$ be a fixed points. Conditioning $X$ on reaching $v$ at a fixed time $T>0$ gives the bridge process $X|X_T=v$. Denoting this process $Y$, Doob's $h$-transform shows that $Y$ is a solution of the SDE (see e.g. \cite{lyons_conditional_1990})
    \begin{equation}
        \begin{split}
        dY_t &=  \tilde b_t(Y_t)dt + \sigma_t(Y_t)d\tilde W_t , \quad Y_0 = x\\
        \tilde b_t(y) &= b_t(y) +  a_t(y) \nabla_y \log p_{T-t}(y,v), \label{eq: doob's transform 2}
        \end{split}\label{eq:doob}
    \end{equation}
where $p_t(\cdot, \cdot)$ denotes the transition density of the diffusion $X$, $a = \sigma \sigma^T$, and where $\tilde W$ is a $d$-dimensional Brownian motion under a changed probability law. 
Doob's $h$-transform is often used to define conditional diffusion processes. 
From a numerical viewpoint, in most cases, the transition density is intractable and therefore direct simulation of \eqref{eq:doob} is not possible. 

If we instead consider a Girsanov transformation of measures to obtain the a system (see, e.g., \cite[Theorem 1]{delyon_simulation_2006})
    \begin{equation}\label{eq: girsanov's sde transform}
    \begin{split}
        dY_t &=  \tilde b_t(Y_t)dt + \sigma_t(Y_t)d\tilde W_t , \quad Y_0 = x\\
        \tilde b_t(y) &= b_t(y) +  \sigma_t(y) h(t,y), 
    \end{split}
    \label{eq: girsanov's sde transform 2}
    \end{equation}
the corresponding change of measure is given by
    \begin{equation}
        \frac{d\Pb^h}{d\Pb}\bigg|_{\cF_t} = e^{\int_0^t h(s,X_s)^T dW_s - \frac{1}{2}\int_0^t \lVert h(s,X_s)\rVert^2 ds}.
    \end{equation}
From \eqref{eq:doob} it is evident that $h(t,x) = \sigma^T \nabla_x \log p_{T-t}(x,v)$ gives the diffusion bridge. However, different choices of the function $h$ can yield processes which are absolutely continuous wrt. to the actual bridges but which can be simulated directly. 

B. Delyon and Y. Hu \cite{delyon_simulation_2006} suggested to use the $h$-function $h(t,x)= \sigma_t^{-1}(x) \nabla_x \log q_{T-t}(x,v)$, where $q$ denotes the transition density density of a standard Brownian motion with mean $v$, i.e., $q_t(x,v) = (2\pi t)^{-d/2}\exp(-\lVert x-v \rVert^2/2t)$. They furthermore proposed a method that would disregard the drift term $b$, i.e.,  $h(t,x) )= \sigma_t^{-1}(x) \nabla_x \log q_{T-t}(x,v) - \sigma_t^{-1}(x)b_t(x)$.
Under certain regularity assumptions on $b$ and $\sigma$, the resulting processes coverge to the target in the sense that $\lim_{t \uparrow T} Y_t = v$, a.s., and for all bounded continuous functions $f$ the conditional expectation is given by
    \begin{equation}
        \E\left[f(X)|X_T=v\right] = C \E\left[f(Y)\varphi(y) \right],
    \end{equation}
where $\varphi$ is a functional of the whole path $Y$ on $[0,T]$, which can easily be simulated. From the construction of the $h$-function, it can be seen that the missing drift term is accounted for in the correction factor $\varphi$. %The suggestion by Delyon and Hu is a popular choice in practice due to its simplicity.

The simulation approach of \cite{delyon_simulation_2006} can be improved by the simulation scheme introduced by Schauer et al. \cite{schauer2017guided}. Here, an $h$-function defined by $h(t,x) = \nabla_x \log \hat p_{T-t}(x,v)$ is suggested, where $\hat p$ denotes the transition density of an auxiliary diffusion process with known transition densities. The auxililary process can for example be linear because closed form solutions of transition densities for linear processes are available. Under the appropriate measure $\Pb^h$, the guided proposal process is a solution to 
    \begin{equation}
        dY_t = b_t(Y_t)dt + a_t(Y_t) \nabla_{x|_{x=X_t}} \log \hat p_{T-t}(x,v)dt + \sigma_t(Y_t)dW_t.
        \label{eq:schauer}
    \end{equation}
Note the factor $a(t,y)$ in the drift in \eqref{eq:doob} which is also present in \eqref{eq:schauer} but not with the scheme proposed by \cite{delyon_simulation_2006}. Moreover, the choice of a linear process grants freedom to model.
For other choices of an $h$-functions see e.g. \cite{marchand2011conditioning,van2017bayesian}.

Marchand \cite{marchand2011conditioning} extended the ideas of Delyon and Hu by conditioning a diffusion process on partial observations at a finite collection of deterministic times. Where Delyon and Hu considered the guided diffusion processes satisfying the SDE
    \begin{equation}\label{eq: delyon hu sde}
        dy_t = b_t(y_t)dt - \frac{y_t-v}{T-t}dt + \sigma_t(x_t)dw_t,
    \end{equation}
for $v \in \R^d$ over the time interval $[0,T]$, Marchand proposed the guided diffusion process conditioned on partial observations ${v_1,\dots, v_N}$ solving the SDE
    \begin{equation}\label{eq: marchand sde}
        dy_t = b_t(y_t)dt - \sum_{k=1}^n P_t^k(y_t)\frac{y_t-u_k}{T_k-t}1_{(T_k - \varepsilon_k,T_k)}dt + \sigma_t(x_t)dw_t,
    \end{equation}
where $u_k$ is be any vector satisfying $L_k(x)u_k = v_k$, $L_k$ a deterministic matrix in $M_{m_k,n}(\R)$ whose $m_k$ rows form a orthonormal family, $P^k_t$ are projections to the range of $L_k$, and $T_k-\varepsilon_k < T_k$. We will only consider the case $k=1$. The requirement that $LY_T = v$ can be interpreted in the sense that $Y_T$ belongs to the preimage of $v$ under $L$, i.e., $Y_T \in L^{-1}(v)$.






==> Content/Sub-content/exp_normal_chart.tex <==
\subsection{Exponential Normal Charts}

The exponential normal chart a parametrization of $M$ that covers all of $M$ except for a subset of volume measure zero. The normal chart provides a linearization of the manifold. Accordingly, the exponential normal chart is a popular choice within geometrical statistics for the aforementioned reasons. 

In this section, we exploit the properties of the normal chart in order to guide the bridges to the diagonal in our simulation scheme. 

Recall that the horizontal stochastic development of an $\R^d$-valued Brownian motion $W$ is a solution to the SDE $dU_t = H_i(U_t) \circ dW^i_t$. The corresponding stochastic development in $M$ is then the solution of the SDE $dX_t = U_t(e_i) \circ dW^i_t$. Choosing any local chart, the Brownian motion in $M$ is a solution to the SDE 
    \begin{equation}\label{eq: local brownian motion}
        dX^i_t = -\frac{1}{2}g^{lk}(X_t)\Gamma^i_{kl}dt + \sigma_j^i(X_t)dW^j_t,
    \end{equation}
where $(g^{ij})_{ij}$ denotes the inverse of the Riemannian metric tensor, $(\Gamma^i_{kl})$ are the Christoffel symbols of the Levi-Civita connection, and $\sigma_j^i = \sqrt{g^{ij}}$. For a detailed derivation of equation \eqref{eq: local brownian motion} consult \cite[Chapter 3]{hsu2002stochastic}.





==> Content/Sub-content/manifold_diffusions.tex <==
\subsection{Manifold-Valued Diffusion Processes}
%The fundamental theorem of stochastic calculus, It\^o's formula, provide the necessary building block for defining stochastic processes on manifolds. It\^o's formula states that the semimartingale property is preserved by $C^2$-transformations. Hence, a natural definition of continuous semimartingales on manifolds is by requiring that $X_t$ is a continuous semimartingales on $M$ if for all smooth functions $f$ on $M$ holds that $f(X_t)$ is a real-valued semimartingale. Although the simplicity in the definition is appealing, the definition is difficult to work with in practice. 



To work with diffusion bridges and guided proposals on manifolds, we will first need to consider the Eells-Elworthy-Malliavin construction of Brownian motion and the connected characterization of semimartingales \cite{elworthy1988geometric}. Endowing the frame bundle $FM$ with a connection allows a splitting of the tangent bundle $TFM$ into a horizontal and vertical part. If the connection on $FM$ is a lift of a connection on $M$, e.g. the Levi-Civita connection of a metric on $M$, the horizontal part of the frame bundle is in one-to-one correspondence with $M$. In addition, there exist fundamental horizontal vector fields $H_i \colon  FM \rightarrow HTFM$ such that for any continuous $\R^d$-valued semimartingale $Z$ the process $U$ defined by
    \begin{equation*}
        dU_t = H_i(U_t) \circ dZ^i_t,
    \end{equation*}
is a horizontal frame bundle semimartingale, where $\circ$ denotes integration in the Stratonovich sense. Let $\pi \colon FM \rightarrow M$ be the bundle projection. The process $X_t := \pi(U_t)$ is then a semimartingale on $M$.
Any semimartingale $X_t$ on $M$ has this relation to a Euclidean semimartingale $Z_t$. $X_t$ is denoted the development of $Z_t$, and $Z_t$ the antidevelopment of $X_t$. We will use this relation when working with bridges on manifolds below.
%satisfying the stochastic differential equation
%    \begin{equation*}
%        dX_t = U_t(e_i) \circ dZ^i_t,
%    \end{equation*}
%which follows from It\^o's formula with $H_i \pi(U_t) = \pi_* (U_t(e_i))^* = U_t(e_i)$ where $(v)^* \in H_uFM$ denotes the horizontal lift of a vector $v \in T_{\pi(u)}M$.
%

When $X_t$ is a Brownian motion, we can also consider coordinate representations of the process. With an atlas $\{(D_{\alpha}, \phi_{\alpha})\}_{\alpha}$ of $M$, there exists an increasing sequence of predictable stopping times $0 \leq T_k \leq T_{k+1}$ such that on each stochastic interval $\llbracket T_k, T_{k+1}\rrbracket = \{(\omega,t)\in \Omega \times \R_+| T_k(\omega) \leq t \leq T_{k+1}(\omega)\}$ the process $x_t \in D_{\alpha}$, for some $\alpha$ (see \cite[Lemma 3.5]{emery1989stochastic}). Thus, the Brownian motion $x$ on $M$ can be described locally in a chart $D_{\alpha} \subset M$ as the solution to the system of SDEs, for $(\omega,t) \in \llbracket T_k, T_{k+1} \rrbracket \cap \{T_k < T_{k+1}\}$
    \begin{equation}\label{eq: local brownian motion}
        dx_t^i(\omega) = b^i(x_t(\omega))dt + \sigma^i_j(x_t(\omega)) dW^j_t(\omega), 
    \end{equation}
where $\sigma$ denotes the matrix square root of the inverse of the Riemannian metric tensor $(g^{ij})$ and $b^k(x) = - \frac{1}{2}g^{ij}(x)\Gamma^k_{ij}(x)$ is the contraction over the Christoffel symbols (see, e.g., \cite[Chapter 3]{hsu2002stochastic}). Strictly speaking, the solution of equation \eqref{eq: local brownian motion} is defined by $x_t^i = \phi_{\alpha}(x_t)^i$. 

Throught the paper, we assume that $M$ is stochastically complete, i.e. long time existence of the Brownian motion and, as a consequence, $\int_M p_t(x,y) d\Vol_M(y) = 1$, for all $t \geq 0$ and all $x \in M$.


==> Content/Sub-content/riemannian_bridges.tex <==



\subsection{Diffusion Bridges on Riemannian Manifolds}\label{sec: bridges on manifolds}

If $p_t$ denotes the transition density of a Brownian motion on $M$, the Brownian bridge process $Y$ on $M$ conditioned at $Y_T = v$ is a Markov process with generator $\frac{1}{2}\Delta + \nabla \log p_{T-t}(\cdot, v)$. Closed form expressions of the transition density of a Brownian motion are available on selected manifolds including Euclidean spaces, hyperbolic spaces, and hyperspheres. Direct simulation of Brownian bridges is therefore possible in these cases. However, generally, transition densities are intractable and auxiliary processes are needed to sample from the desired conditional distributions.  

To this extend, various types of bridge processes on Riemannian manifolds have been described in the literature. In case of manifolds with a pole, i.e, the existence of a point $p \in M$ such that the exponential map $\exp_p \colon T_pM \rightarrow M$ is a diffeomorphism, the \textit{semi-classical} (Riemannian Brownian) bridge was introduced by Elworthy and Truman \cite{elworthy1982diffusion} as the process with generator $\frac{1}{2}\Delta + \nabla \log k_{T-t}(\cdot, v)$, where
    \begin{equation*}
        k_t(x,v) = (2\pi t)^{-n/2} e^{-\frac{d(x,v)^2}{2t}} J^{-1/2}(x),
    \end{equation*}
and $J(x) = |\det D_{\exp(v)^{-1}} \exp_{v}|$ denotes the Jacobian determinant of the exponential map at $v$. Elworthy and Truman used the semi-classical bridge to obtain heat kernel estimates and the semi-classical bridge has been studied by various others \cite{li2017semi,ndumu1991brownian}. 

By Varadhan's result (see \cite[Theorem 5.2.1]{hsu2002stochastic}), as $t \rightarrow T$, we have the asymptotic relation $((T-t) \log p_{T-t}(x,y) \sim  -\frac{1}{2}d(x,y)^2$. In particular, the following asymptotic relation was shown to hold by Malliavin, Stroock, and Turetsky \cite{malliavin1996short,stroock1997short} : $(T-t)\nabla \log p_{T-t}(x,y) \sim - \frac{1}{2} \nabla d(x,y)^2$. From these results it is seen from their generators that the Brownian bridge and the semi-classical bridge differ in the limit by a factor of $-\frac{1}{2}\nabla \log J(x)$. However, under a certain boundednes condition the two processes can be shown to be identical under a changed probability measure \cite[Theorem 4.3.1]{thompson2015submanifold}.

In order to generalize the heat-kernel estimates of Elworthy and Truman, Thompson \cite{thompson2015submanifold,thompson2018brownian} considered the \textit{Fermi} bridge process conditioned to arrive in a submanifold $N \subseteq M$ at time $T>0$. The Fermi bridge is defined as the diffusion process with generator $\frac{1}{2}\Delta + \nabla \log q_{T-t}(\cdot, N)$, where
    \begin{equation*}
        q_t(x,N) = (2\pi t)^{-n/2} e^{-\frac{d(x,N)^2}{2t}}.
    \end{equation*}
True for both of these bridge processes is, that when $M = \R^d$ and $N$ is a point both the semi-classical bridge and the Fermi bridge agree with the Euclidean Brownian bridge. In particular, the Fermi bridge provides a method on which to condition on subsets of the original space. 


In \cite{jensen2021simulation}, the authors introduced a numerical simulation scheme of conditioned diffusions on Riemannian manifolds which generalized the method by Delyon and Hu \cite{delyon_simulation_2006} to manifolds. The guiding term used is identical to the guiding term of the Fermi bridge when the submanifold is a single point $v$.

==> Content/Sub-content/riemannian_geometry.tex <==
\subsection{Riemannian Geometry}

%\subsubsection{Preliminaries to Riemannian Geometry --} In this section, core concepts of differential and particularly Riemannian geometry are introduced. 
A Riemannian manifold of dimension $d$ is a pair $(M, g)$ consisting of a differentiable manifold $M$ of dimension $d$ endowed with a Riemannian metric $g$, i.e. a family of innner products $(g_p)_{p \in M}$ on each tangent space $T_p M$ varying smoothly in $p$. Throughout, we also refer to $M$ as the Riemannian manifold when the metric is understood or simply just as the manifold without emphasis on differentiability. The Riemannian metric allows for geometric definitions of, e.g., length of curves, angles of intersections, and volumes on manifolds. A differentiable curve on $M$ is a map $\gamma \colon [0,1] \rightarrow M$ for which the time derivative $\gamma'(t)$ belongs to $T_{\gamma_t}M$, for each $t \in (0,1)$. The length of the differentiable curve can then be determined from the Riemannian metric by $L(\gamma) := \int_0^1 \sqrt{g_{\gamma_t}\left(\gamma'(t), \gamma'(t)\right)} dt = \int_0^1 \lVert \gamma'(t) \rVert_{\gamma_t} dt$. Let $p,q \in M$ and let $\Gamma$ be the set of differentiable curves joining $p$ and $q$, i.e., $\Gamma = \{\gamma \colon [0,1] \rightarrow M | \gamma(0) = p$ and $\gamma(1) =q\}$. The (Riemannian) distance between $p$ and $q$ is defined as $d(p,q) = \min_{\gamma \in \Gamma} L(\gamma)$. Instead of minimizing over $\Gamma$, we could instead minimize over the subset $\Gamma^0 \subset \Gamma$ consisting of those curves with constant speed, i.e., $\lVert \gamma'(t)\rVert_{\gamma_t} = c$ for some constant $c > 0$. Minimizing curves are called \textit{geodesics}.

A manifold can be parameterized using coordinate charts. These charts consists of open subsets of $M$ providing a global cover of $M$ and such that each subset is diffeomorphic to an open subset of $\R^d$. %This is an intrinsic description of a manifold which shows its local Euclidean structure. Alternatively, Whitney's embedding theorem states that any (smooth) manifold can be embedded into a higher dimensional Euclidean space. A classical example of Whitney's embedding is the $2$-sphere centered at the origin of $\R^3$. 
The exponential normal chart is often a convenient choice to parameterize a manifold for computational purposes. The exponential chart is related to the exponential map $\exp \colon TM \rightarrow M$, where $TM$ denotes the tangent bundle, i.e., a collection of pairs $(p,v) \in M \times T_pM$, for every $p \in M$. Equivalently, the exponential map, for each $p\in M$, as $\exp_p \colon T_pM \rightarrow M$ is given by $\exp_p(v) = \gamma_v(1)$, where $\gamma_v$ is the unique geodesic satisfying $\gamma_v(0)=p$ and $\gamma_v'(0) = v$. For each $p \in M$, the tangent map is a diffeomorphism from a star-shaped subset $V$ centered at the origin of $T_pM$ to its image $\exp_p(V) \subseteq M$, covering all of $M$ except for a subset of (Riemannian) volume measure zero $\Cut(p)$ called the \textit{cut-locus of $p$}. The inverse map $\log_p \colon M\backslash \Cut(p) \rightarrow T_pM$ provides a local parameterization of $M$ due to the isomorphism between $T_pM$ and $\R^d$.

Closely related to the tangent bundle is the frame bundle $FM$, which for each point $p \in M$ assigns a frame or basis for the tangent space $T_pM$, i.e., $FM$ consists of a collection of pairs $(p,u)$, where $u \colon \R^d \rightarrow T_pM$ is a linear isomorphism. There exist a subbundle of $FM$ consisting of orthonormal frames called the orthonormal frame bundle $OM$. In this case, the map $u \colon \R^d \rightarrow T_pM$ is a linear isometry.



==> Content/Sub-content/wDM.tex <==
\subsection{Weighted Diffusion-Mean}
%In manifolds where geodesics cannot be found from a closed-form solution, it becomes a computationally heavy task to evaluate the weighted Fréchet mean in each convolutional layer of the network. Instead, the weighted Fréchet mean can be exchanged with a weighted diffusion-$t$-mean.
The diffusion-mean was introduced as geometric mean satisfying the probabilistic property of the Euclidean expected value, specifically as the starting point of Brownian motion which is most likely given observed data \cite{hansen2021diffusiongeometric, hansen2021diffusion}. This results in the \textit{diffusion $t$-mean} definition
    \begin{equation}
        \mu_t = \argmin_{p\in M} \E\left[ - \log p_{t}(p,X) \right],
    \end{equation}
where $p_t(\cdot, \cdot)$ denotes the transition density of a Brownian motion on $M$. Equivalently, $p_t$ denotes the solution to the heat equation $\partial u/ \partial t = \Delta_g u$, where $\Delta_g$ denotes the Laplace-Beltrami operator associated with the Riemannian metric $g$. 
The definition allows for an interpretation of the mean as an extension of the Fréchet mean due to Varadhan's result stating $\lim_{t \downarrow 0}-2 t \log p_t(x,y) =  d(x,y)^2$ uniformly on compact sets disjoint from the cut-locus of either $x$ or $y$ \cite{hsu2002stochastic}.

Just as the Fr\'echet mean, the diffusion mean has a weighted version, and the corresponding estimator of the \textit{weighted} diffusion $t$-mean is given as
    \begin{equation}
        \hat \mu_t =  \argmin_{p \in M}  \sum_{i=1}^n - \log p_{t/w_i}(p,x_i).
        \label{eq:wdiffusionmean}
    \end{equation}
     
As closed form expressions for the heat kernel are only available on specific manifolds, evaluating the diffusion-$t$-mean often my rely on numerical methods. 
One example of this is bridge sampling that allows to numerically estimate the transition density of a diffusion process using guided proposal schemes. If a global coordinate chart is available, the transition density can be written in the form (see \cite{papaspiliopoulos2012importance, jensen2021simulation})
    \begin{equation}\label{eq: transition density estimate}
        p_T(z,v) = \sqrt{\frac{\det A(v)}{(2\pi T)^2}}e^{- \frac{\lVert a(z)(z-v)\rVert^2}{2T}} \E\left[\varphi_T\right],
    \end{equation}
where $a$ is the matrix square root of $A$ and $\varphi$ denotes the correction factor between the law of the true diffusion bridge and the law of the guided proposal scheme. The expectation over the correction factor can be numerically approximated using Monte Carlo sampling. We detail the setup further below.

==> Content/Sub-content/wFM.tex <==
\subsection{Weighted Fréchet Mean}

The most fundamental statistic is the sample mean estimator, which in Euclidean space is given by the arithmetic mean. Moreover, the Euclidean mean has three defining properties: The \textit{algebraic property} states the uniqueness of the arithmetic mean as the mean with residuals summing to zero, the \textit{geometric property} defines the mean as the point that minimizes the variance, and the \textit{probabilistic property} adheres to a maximum likelihood principle given an i.i.d. assumption on the observations (see also \cite[Chapter 2]{pennec2019riemannian}).



Direct generalization of the arithmetic mean to non-linear spaces is in general not possible due to the vector space structure. However, the defining properties above allow to give candidate definitions of mean values in non-linear spaces. %The geometric property, i.e., the arithmetic mean is the value which minimize the sum of squared distances, generalizes to various metric spaces. 

The Fréchet mean \cite{frechet1948elements} uses the geometric property by generalization the mean-squared distance minimization property to general metric spaces. Given a random variable $X$ on a metric space $(E,d)$, the Fréchet mean is defined by
    \begin{equation}\label{eq: frechet mean}
        \mu = \argmin_{p \in E} \E\left[d(p,X)^2 \right].
    \end{equation}
Here, the metric space is a Riemannian manifold $M$ with Riemannian distance function $d$. Given realizations $x_1,\dots, x_n \in M$ from a distribution on $M$, the estimator of the \textit{weighted} Fréchet mean is defined as
    \begin{equation}\label{eq: weighted frechet mean}
        \hat \mu = \argmin_{p \in M} \sum_{i = 1}^n w_i d(p, x_i)^2,
    \end{equation}
where $w_1, \dots, w_n$ are the corresponding weights satisfying $w_i > 0$ and $\sum_i w_i = 1$. When the weights are identical, \eqref{eq: weighted frechet mean} is the estimator for the Fréchet mean. Throughout, we shall make no distinction between the estimator and the Fréchet mean and will refer to both as the Fréchet mean.



In \cite{chakraborty2018manifoldnet,chakraborty2020manifoldnet}, the weighted Fréchet mean was introduced to define a generalization of the Euclidean convolution to manifold-valued inputs. When closed-form solutions of geodesics are available, the weighed Fre\'echet mean can be estimated efficiently with a recursive algorithm also denoted an inductive estimator.

==> Content/numerical_experiments.tex <==
%\section{Numerical Experiments}

\iffalse

\begin{figure}[h]
        \centering
    \begin{subfigure}[t]{0.325\textwidth}
    \centering
        \includegraphics[width=0.8\linewidth]{Figures/Mean_on_diagonal_S2.png}
        \label{fig: Mean on diagonal of S2 north pole}
    %\caption{}\label{fig: north pole}
    \end{subfigure}
    \hfill
    \centering
    \begin{subfigure}[t]{0.325\textwidth}
    \centering
        \includegraphics[width=0.8\linewidth]{Figures/mean_on_diagonal_S2_south_pole.png}
        \label{fig: Mean on diagonal of S2 south pole}
    %\caption{}\label{fig: south pole}
    \end{subfigure}
    \hfill
    \centering
    \begin{subfigure}[t]{0.325\textwidth}
    \centering
        \includegraphics[width=0.8\linewidth]{Figures/Mean_on_diagonal_S2_antipodal.png}
        \label{fig: Mean on diagonal of S2 south pole}
    %\caption{}\label{fig: antipodal}
    \end{subfigure}
    \caption{Convergence of a stochastic system of equations on the product manifold of $\mathbb S^2$ conditioned to arrive at the diagonal visualized here on $\mathbb S^2$. The cyan-colored dot indicate the Frechét estimate of the given observations. The piece-wise curve (beige) indicate the moving average on the diagonal, initialized from the north pole (left), south pole (middle), and antipodal of the Fréchet mean (right), respectively.}
\end{figure}

\fi



\begin{figure}[ht]
     \centering
    \begin{subfigure}[t]{0.48\textwidth}
    \centering
        \includegraphics[width=0.75\linewidth]{Figures/bridge_on_diagonal_with_frechet_mean.png}
           %\caption{}\label{fig: south pole}
    \end{subfigure}
    \hfill
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
    \centering
        \includegraphics[width=0.75\linewidth]{Figures/data_on_s2_with_frechet_mean_1.png}
    %\caption{}\label{fig: south pole}
    \end{subfigure}
    \caption{100 data points from a von Mises-Fisher distribution with $\kappa = 2$ and $\mu = (0,0,1)$. The Fréchet-mean (cyan dot) is calculated using gradient-descent based optimization whereas the diffusion-mean (blue) is approximated using bridge sampling in $\mathbb S^{2n}:= \mathbb S^2 \times \cdot \mathbb S^2$ conditioned on the diagonal.}\label{fig: Mean on sphere}
\end{figure}


==> Definitions/journalnames.tex <==
%%Updated on 15 January 2022
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}\gdef\@continuouspages{yes}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{CTN}\gdef\@doiabbr{Clin. Transl. Neurosci.}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharm.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kidneydial}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-coding RNA}\gdef\@journalshort{Non-coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}

